A Long Horizon Planning Framework for Manipulating Rigid Pointcloud Objects

We present a framework for solving long-horizon planning problems involving manipulation of rigid objects that operates directly from a point-cloud observation, i.e. without prior object models. Our method plans in the space of object subgoals and frees the planner from reasoning about robot-object interaction dynamics by relying on a set of generalizable manipulation primitives. We show that for rigid bodies, this abstraction can be realized using low-level manipulation skills that maintain sticking contact with the object and represent subgoals as 3D transformations. To enable generalization to unseen objects and improve planning performance, we propose a novel way of representing subgoals for rigid-body manipulation and a graph-attention based neural network architecture for processing point-cloud inputs. We experimentally validate these choices using simulated and real-world experiments on the YuMi robot. Results demonstrate that our method can successfully manipulate new objects into target configurations requiring long-term planning. Overall, our framework realizes the best of the worlds of task-and-motion planning (TAMP) and learning-based approaches. Project website: https://anthonysimeonov.github.io/rpo-planning-framework/.

==> figText/cylinder.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{sample_figures/mustard_many_tight_2.png}    
    \caption{\small {\bf Top} Predictions made from pointclouds of objects of novel geometric classes, by our model which was only trained on cuboids. {\bf Bottom} Executing a plan found for a 3-step plan skeleton on a bottle-shaped object}
    \label{fig: cylinders}
    \vspace{-15pt}
\end{figure}

==> figText/gat_v_pointnet_grasps.tex <==
\begin{wrapfigure}{r}{.6\linewidth}
    \centering
    \includegraphics[width=\linewidth]{sample_figures/gat_vs_pointnet_samples_thin.png}    
    \caption{Qualitative examples of typical $T^p$ predictions from our GAT-based model and PointNet++-based model. Our architecture provides a large benefit in predicting palm poses that make a sticking patch contact and are aligned to the object orientation.}
    \label{fig: grasp_motion_plan}
\end{wrapfigure}

==> figText/mustard_multi.tex <==
\begin{wrapfigure}{r}{.6\linewidth}
    \centering
    \includegraphics{sample_figures/mustard_many_tight_0.png}
    \caption{Mustard bottle}
    \label{fig:mustard-multi}
\end{wrapfigure}

==> figText/pose_unstable.tex <==
\begin{wrapfigure}{r}{.3\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/grasp_unstable.pdf}
    \caption{Examples of what oftentimes happens when directly sampling $T^o$ from the trained decoder when using the grasping skill. Object can penetrate the table, float in the air, be tilted in an unstable configuration, or some combination of all.} 
    \label{fig: pose_unstable}
\end{wrapfigure}

==> figText/pybullet_rows.tex <==
\begin{wrapfigure}{r}{.3\linewidth}
    \centering
    \includegraphics[width=\linewidth]{sample_figures/pybullet_rows_labeled.png}
    \caption{Snapshots during the execution of a (top) pull, (middle) grasp, and (bottom) push skills on the simulated YuMi robot in PyBullet.} 
    \label{fig: real-pcd}
\end{wrapfigure}

==> figText/real_pcd.tex <==
\begin{wrapfigure}{r}{.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{sample_figures/real_pcd_all_skills_0.png}    
    \caption{Visualization of predicted contact poses of the manipulator with real pointcloud objects for different skills.}
    \label{fig: real-pcd}
    \vspace{-10pt}
\end{wrapfigure}
